Multimodal Pretraining, Adaptation, and Generation for Recommendation: A Survey

Personalized recommendation serves as a ubiquitous channel for users to discover information tailored to their interests. However, traditional recommendation models primarily rely on unique IDs and categorical features for user-item matching, potentially overlooking the nuanced essence of raw item contents across multiple modalities such as text, image, audio, and video. This underutilization of multimodal data poses a limitation to recommender systems, especially in multimedia services like news, music, and short-video platforms. The recent advancements in large multimodal models offer new opportunities and challenges in developing content-aware recommender systems. This survey seeks to provide a comprehensive exploration of the latest advancements and future trajectories in multimodal pretraining, adaptation, and generation techniques, as well as their applications in enhancing recommender systems. Furthermore, we discuss current open challenges and opportunities for future research in this dynamic domain. We believe that this survey, alongside the curated resources, will provide valuable insights to inspire further advancements in this evolving landscape.

==> Content/CCS.tex <==
\begin{CCSXML}
<ccs2012>
  <concept>
      <concept_id>10002951.10003317.10003347.10003350</concept_id>
      <concept_desc>Information systems~Recommender systems</concept_desc>
      <concept_significance>500</concept_significance>
  </concept>
 </ccs2012>
\end{CCSXML}
\ccsdesc[500]{Information systems~Recommender systems}

==> Tables/paper-list.tex <==
\definecolor{deepgreen}{RGB}{45,120,45}
\definecolor{deepblue}{RGB}{45,45,120}
\definecolor{deepred}{RGB}{120,45,45}
\definecolor{deepyellow}{RGB}{120,120,45}
\definecolor{deeppurple}{RGB}{120,45,120}
\definecolor{deepcyan}{RGB}{45,120,120}

\newcommand{\PDt}{\keyboardkey{text}{deepgreen}}
\newcommand{\PDa}{\keyboardkey{aural}{deepblue}}
\newcommand{\PDv}{\keyboardkey{visual}{deepred}}
\newcommand{\PDb}{\keyboardkey{behavior}{deepyellow}}
\newcommand{\PDp}{\keyboardkey{profile}{deeppurple}}
\newcommand{\PDi}{\keyboardkey{interaction}{deepcyan}}

\begin{table*}[]
\renewcommand\arraystretch{1.2}

\begin{tabular}{c|c|c|c|c|c|c}
\toprule
\textbf{Paper} & \textbf{Venue} & \textbf{Pretrain} & \textbf{Paradigm} & \textbf{Modality} & \textbf{Adaption}  & \textbf{Domain}\\
\midrule
PREC~\cite{prec} & COLING'22 & post & Predictive & \PDt \sep \PDb \sep \PDp & Representation & News \\
ONCE~\cite{once} & WSDM'24 & general & Generative & \PDt & Prompting & Content-based \\
P5~\cite{p5} & RecSys'22 & post & Generative & \PDt & Prompting & Text-based \\
Bert4Rec~\cite{bert4rec} & CIKM'19 & in & Predictive & \PDb & Generation & Sequential \\
FANS~\cite{fans} & WWW'23 & in & Predictive & \PDb & Generation  & Sequential \\
CAGE~\cite{cage} & WWW'24 & in & Predictive & \PDb & Generation & Sequential \\
UserBERT~\cite{userbert} & SIGIR'22 & in & Contrastive;Predictive & \PDb & Finetune & Sequential \\
PLM-NR~\cite{plm-nr} & SIGIR'21 & general & Predictive & \PDt & Finetune & News \\
PeterRec~\cite{peterrec} & SIGIR'20 & in & Generative & \PDb & Finetune & Cross-domain \\
S3-Rec~\cite{s3rec} & SIGIR'20 & in & Predictive & \PDt \sep \PDb \\
SL4Rec~\cite{sl4rec} & CIKM'21 & in & Contrastive & \PDt \\
UniSRec~\cite{unisrec} & KDD'22 & in & Contrastive & \PDt \sep \PDb \\
RecFormer~\cite{recformer} & KDD'23 & in & Predictive;Contrastive & \PDt \sep \PDb \\
P5~\cite{p5} & RecSys'22 & in & Generative & \PDt \sep \PDb \\
MMSSL~\cite{mmssl} & WWW'23 & in & Contrastive & \\
\bottomrule

\end{tabular}
\end{table*}

